TotalDefMeme: A Multi-Attribute Meme dataset on Total Defence in Singapore

Total Defence is a defence policy combining and extending the concept of military defence and civil defence. While several countries have adopted total defence as their defence policy, very few studies have investigated its effectiveness. With the rapid proliferation of social media and digitalisation, many social studies have been focused on investigating policy effectiveness through specially curated surveys and questionnaires either through digital media or traditional forms. However, such references may not truly reflect the underlying sentiments about the target policies or initiatives of interest. People are more likely to express their sentiment using communication mediums such as starting topic thread on forums or sharing memes on social media. Using Singapore as a case reference, this study aims to address this research gap by proposing TotalDefMeme, a large-scale multi-modal and multi-attribute meme dataset that captures public sentiments toward Singapore's Total Defence policy. Besides supporting social informatics and public policy analysis of the Total Defence policy, TotalDefMeme can also support many downstream multi-modal machine learning tasks, such as aspect-based stance classification and multi-modal meme clustering. We perform baseline machine learning experiments on TotalDefMeme and evaluate its technical validity, and present possible future interdisciplinary research directions and application scenarios using the dataset as a baseline.

==> Analysis.tex <==
Coming soon...

==> Total-Defence.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.8]{images/data-annotation-pipeline.pdf}
    \caption{Data Collection \& Annotation Pipeline. The annotations in the figure is based on the example meme in Figure \ref{fig:example}.}
    \label{fig:data-annotation-pipeline}
\end{figure*}

The Total Defence policy is a defence policy that incorporates both military and civil defence strategies. It is adopted by countries such as Finland, Norway, Sweden, and Singapore. The policy emphasizes a high level of readiness against any potential dangers and catastrophes, including war, crisis, and natural disasters, for the state and its society. Hence, as a key defence policy, Total Defence serves as the primary guide to the needs of the government and its citizens.

\textbf{Singapore’s Total Defence.} While various countries employ the Total Defence policy, their implementation is not globally uniform.  Our research involved collecting and analyzing memes pertaining to Singapore's Total Defence policy, which comprises six pillars: Military Defence, Civil Defence, Economic Defence, Social Defence, Psychological Defence, and Digital Defence. Through our examination of multiple sources\footnote{https://www.mindef.gov.sg/oms/imindef/mindef\_websites/topics/totaldefence/about.html}\footnote{https://www.scdf.gov.sg/home/community-volunteers/community-preparedness/total-defence}, we have summarized the definitions of each pillar in the following abstracts:

\begin{itemize}

\item \textbf{Military Defence}: Strong and formidable defence force made up of Regulars and National Servicemen, and supported by the entire nation
\item \textbf{Civil Defence}: Collective effort of the society to spot signs of threats, respond effectively and recover quickly from crisis
\item \textbf{Economic Defence}: Strong and resilient economy that is globally competitive and able to bounce back from any crisis.
\item \textbf{Social Defence}: Bonds that unite us, built on trust and understanding among people of different race and religions, living in harmony and looking out for one another
\item \textbf{Psychological Defence}: The will and resolve to defend our way of life and interests, the fighting spirit to overcome challenges together
\item \textbf{Digital Defence}: Being secure, alert and responsible online.
\end{itemize}
